Cost-Effective Proxy Reward Model Construction with On-Policy and Active Learning

Reinforcement learning with human feedback (RLHF), as a widely adopted approach in current large language model pipelines, is \textit{bottlenecked by the size of human preference data}. While traditional methods rely on offline preference dataset constructions, recent approaches have shifted towards online settings, where a learner uses a small amount of labeled seed data and a large pool of unlabeled prompts to iteratively construct new preference data through self-generated responses and high-quality reward/preference feedback. However, most current online algorithms still focus on preference labeling during policy model updating with given feedback oracles, which incurs significant expert query costs. \textit{We are the first to explore cost-effective proxy reward oracles construction strategies for further labeling preferences or rewards with extremely limited labeled data and expert query budgets}. Our approach introduces two key innovations: (1) on-policy query to avoid OOD and imbalance issues in seed data, and (2) active learning to select the most informative data for preference queries. Using these methods, we train a evaluation model with minimal expert-labeled data, which then effectively labels nine times more preference pairs for further RLHF training. For instance, our model using Direct Preference Optimization (DPO) gains around over 1% average improvement on AlpacaEval2, MMLU-5shot and MMLU-0shot, with only 1.7K query cost. Our methodology is orthogonal to other direct expert query-based strategies and therefore might be integrated with them to further reduce query costs.

==> intro_archive.tex <==
\section{Introduction}
\yf{Still too long, need to rewrite}
Reinforcement learning from human feedback (RLHF) has gained significant attention in recent years. One traditional direction, exemplified by Proximal Policy Optimization (PPO) and its variants \citet{ouyang2022training,swamy2024minimaximalist}, maintains one or several standalone reward models to finetune the policy model online by maximizing the rewards. Another approach involves directly optimizing preference data without using an explicit reward model, as seen in offline Direct Preference Optimization (DPO)  and its variants \cite{rafailov2024direct, azar2024general, rosset2024direct, wu2024SPO}. Recently, hybrids methods have been used in \cite{yuan2024selfreward, dong2024rlhf, wu2024SPO, viethoangtranduong} that combines the flexibility of the first approach with the training stability of the second by using standalone reward models as proxy feedback oracles to label preference data. Our work explores this \textit{hybrid} setting, focusing specifically on how to efficiently \textit{train such reward models with minimal expert queries}.

\begin{figure*}[!h]
    \centering
    \setlength{\belowcaptionskip}{-20pt} % Adjust this value as needed
    \includegraphics[scale=0.6]{figures/pipeline.png}
    \caption{Our cost-effective preference data labeling pipeline. \yf{TODO}}
    \label{fig:pipeline}
\end{figure*}

Many RLHF methods suffer from the \textit{scarcity of human preference labeled data}. Classic works such as \citet{bai2022training,cui2023ultrafeedback, zhu2023starling} aim to build high-quality, model-independent datasets offline. However, these methodologies primarily focus on data quality without considering the informativeness of the samples relative to the target model. This oversight can lead to distribution shifts issues when the training model differs from the exploratory models used to generate the dataset.
% For example, if we have an standalone reward model trained on those data, then the newly generated responsed from our training mode can easily fall into the out-of-distrbution (OOD) domain. If we are using DPO training, then we may waste resources on optimizing on some already good domain. 

To address these challenges, recent research has shifted focus to online self-improvement techniques, also referred to as "on-policy" or "iterative" methods. These methods leverage a set amount of labeled seed data and a large pool of unlabeled prompts, with the goal of continuously improving the model through responses generated by the model itself, and potentially, through external reward feedback. The primary expense in this process is \textit{the cost of expert reward queries}. To conserve the query budget, researchers have developed three main categories of strategies. The first category, represented by Self-play Finetuning (SPIN) \cite{wang2023self}, eliminates the need for reward feedback by utilizing initial supervised finetuning data. The second category, which is the \textit{focus of our work}, aims to reduce expert queries during the construction of the proxy oracle. The self-reward framework \cite{yuan2024selfreward} can be partially included in this category as we will discussed later. The third category focuses on improving the efficiency of direct preference queries through either online batch query strategies or advanced exploratory policies, regardless of the type of oracle used. \cite{rosset2024direct,xiong2023iterative,dong2024rlhf, viethoangtranduong, wu2024SPO} If the oracle is an expert, this is equivalent to reducing the expert query cost. On the other hand, when using proxy reward oracles, the main cost shifts towards optimizing the construction of these oracles. This brings us back to the concerns of the second category.

\textit{The first and third categories (assuming using expensive expert oracle), however, still demand a significant amount of labeled data. } Specifically, SPIN requires a substantial number of ground truth responses to be positive samples in preference pairs, as a trade-off of eliminating reward feedback. Meanwhile, online direct preference demands extensive querying for expert preference/reward oracle. Conversely, \textit{how to saving the cost when constructing the proxy reward oracle, is still under-explored.} Some studies \cite{dong2024rlhf, viethoangtranduong} demonstrate that a proxy reward oracle trained on a smaller model, such as PairRM 0.4B \citet{jiang2023llm}, can effectively replace more robust experts like GPT-3. Nonetheless, the development of such models still demands substantial external resources, including offline data for training the reward model and benchmark data for testing and selecting the appropriate reward model.

Inspired by the success of proxy reward oracles, we hypothesize that a\textit{ smaller dataset is sufficient} to train a weak evaluation model that can effectively label a much larger set of preference data. Furthermore, inspired by the successes of online methods in the third category, we aim to incorporate on-policy query techniques into the training of evaluation models.

In this paper, we focus on self-improvement under extremely constrained conditions, \textit{where only a limited amount of labeled seed data and a small expert query budget are available—for instance.} (e.g. Seed data is 20 times smaller than many existing works, and the query budget is on the same order as the seed data.) Our objective is not to develop a new state-of-the-art model but to propose a methodology under these stringent conditions that can potentially be combined with other methods.

The most closely related work to our approach is the self-reward pipeline \cite{yuan2024selfreward}, where the focus is also on using a small amount of labeled seed data. However, their approach primarily exploits the intrinsic capability of the model itself without any reward feedback. While this sounds attractive, their methods are not directly comparable to ours as they require an additional powerful model (e.g., Llama2-70B-chat) to generate instructions online instead of using a fixed pool of instructions, which incurs extra query costs. Additionally, their approach heavily relies on the strength of the initial model (e.g., Llama2-70B) and the characteristics of the seed data, which we will demonstrate is not universally applicable even when adapted to our settings.

\begin{figure*}[!h]
    \centering
    \setlength{\belowcaptionskip}{-20pt} % Adjust this value as needed
    \includegraphics[scale=0.6]{figures/pipeline_previouswork.png}
    \caption{Previous preference data labeling pipeline. \yf{TODO}}
    \label{fig: pipeline_previous}
\end{figure*}

\textbf{Our contributions:}
\begin{itemize}[leftmargin=*, itemsep=-2pt, before=\vspace{-8pt}, after=\vspace{-6pt}]
    \item We first propose a random on-policy expert query strategy for labeling the preference data used to train the proxy reward oracle. Our empirical study validates that a weak evaluation model trained with a small amount of data (i.e., a query budget of 1.7K) is capable of effectively labeling up to nine times more preference pairs. For instance, DPO training on Llama-2 7B with 15K preference pairs labeled by us yields a greater than 1\% increase in performance on AlpacaEval2 and MMLU 5-shot metrics compared to the initial supervised finetuning model.
    \item Building on the success of the on-policy approach, we further explore replacing the random query strategy with coreset-type (e.g., \(k\)-center) active learning strategies, to select the most informative prompts and responses from the large unlabeled. Our active learning strategy results in additional performance gains of 0.34\% to 0.6\% on the MMLU-5shot and 0.4\% to 0.53\% on MMLU-shot metrics under a properly managed budget.
    \item Lastly, we compare our method with two existing approaches—SPIN and a seed data query strategy derived from the self-reward paper. We find that SPIN underperforms significantly when only a small amount of seed data is available. Conversely, while the seed data query strategy shows some advantages under extremely low query budgets (e.g., 500), it is quickly outperformed by our proposed methods as the budget increases.
\end{itemize}


